Mesh2NeRF: Direct Mesh Supervision for Neural Radiance Field Representation and Generation

We present Mesh2NeRF, an approach to derive ground-truth radiance fields from textured meshes for 3D generation tasks. Many 3D generative approaches represent 3D scenes as radiance fields for training. Their ground-truth radiance fields are usually fitted from multi-view renderings from a large-scale synthetic 3D dataset, which often results in artifacts due to occlusions or under-fitting issues. In Mesh2NeRF, we propose an analytic solution to directly obtain ground-truth radiance fields from 3D meshes, characterizing the density field with an occupancy function featuring a defined surface thickness, and determining view-dependent color through a reflection function considering both the mesh and environment lighting. Mesh2NeRF extracts accurate radiance fields which provides direct supervision for training generative NeRFs and single scene representation. We validate the effectiveness of Mesh2NeRF across various tasks, achieving a noteworthy 3.12dB improvement in PSNR for view synthesis in single scene representation on the ABO dataset, a 0.69 PSNR enhancement in the single-view conditional generation of ShapeNet Cars, and notably improved mesh extraction from NeRF in the unconditional generation of Objaverse Mugs.

==> AuthorKit/sections_eccv/4results_eccv-.tex <==
\section{Results}
We illustrate that our direct supervision of radiance fields from meshes significantly improves performance in NeRF optimization and generation tasks.
We showcase results of a single scene fitting using Mesh2NeRF, comparing it with NeRF pipelines in Section~\ref{subsec:single_scene_fitting}. Importantly, we then demonstrate the utility of Mesh2NeRF in diverse 3D generation tasks in Section~\ref{subsec:cond_generation} and Section~\ref{subsec:uncond_generation}.


\begin{figure*}[tb!]
\vspace{-0.08in}
\centering
\includegraphics[width=1\textwidth]{AuthorKit/figures/visual_single_obj_scene.pdf}
\vspace{-0.23in}
\caption{Comparison of single scene fitting for scenes from Poly Haven and Sketchfab.  
For each visualized scene, we present two renderings of test views by each method.
Our results showcase higher accuracy and a superior ability to capture finer details in renderings when compared to the baseline methods (Mesh2NeRF~TensoRF vs. TensoRF and Mesh2NeRF~NGP vs. Instant~NGP).
}
\vspace{-0.15in}
\label{fig:vis_vsnerf}
\end{figure*}

\subsection{Single Scene Fitting}
\label{subsec:single_scene_fitting}
This section compares \OURS with traditional NeRF methods in representing a single scene via a neural network. \OURS directly supervises the neural network from mesh data, while traditional NeRFs use rendering technologies and then fuses information from renderings to the radiance field.

We evaluate our method on scenes from Amazon Berkeley Objects (ABO) \cite{collins2022abo}, Poly Haven Models~\cite{polyhaven} and Sketchfab Scenes~\cite{skatchfab}. 
The ABO dataset contains twelve realistic 3D models of household objects. 
Each object is rendered at 512$\times$512 pixels from viewpoints sampled on a sphere, covering the object's surface area (90 views as input and 72 for testing). 
We also show results on six hyper-real models from the Poly Haven library, which consists of quality content designed by artists. Each scene is rendered at 512$\times$512 with 90 input and 120 test views.
We use the \textit{Entrée du château des Bois Francs} scene from Sketchfab to evaluate large scene-scale data. The used Sketchfab scene is also rendered at 512$\times$512 pixels with 90 input views and 120 test views.
For \OURS, we use the textured mesh from both sets by setting a fixed point light. 
We evaluate our approach with three different encodings and parametric data structures for storing trainable feature embeddings, \ie, the network part of NeRFF~\cite{mildenhall2021nerf}, TensoRF~\cite{chen2022tensorf}, and Instant NGP~\cite{muller2022instant} with our \OURS direct supervision using the corresponding mesh. We denote these three methods by Mesh2NeRF NeRF, Mesh2NeRF TensoRF, and Mesh2NeRF NGP, respectively.

In Table~\ref{tab:single_object_results}, we report mean PSNR/SSIM (higher is better) and LPIPS (lower is better) for objects in both the ABO and Poly Haven datasets. 
Our method consistently outperforms prior work on both datasets. 
For the ABO dataset, all three variants of our method surpass baseline optimization across all evaluation metrics. 
Mesh2NeRF NGP, employing Instant NGP style multi-resolution hash table encodings, achieves the best performance. 
Compared to the raw Instant NGP version, Mesh2NeRF NGP exhibits notable improvements ($+3.12$ PSNR, $+0.041$ SSIM, and $-0.021$ LPIPS). 
Similarly, on the Poly Haven dataset, Mesh2NeRF NGP delivers the best results.%, showcasing improvements over Instant NGP (+0.91 PSNR, +0.046 SSIM, and -0.056 LPIPS).

We present qualitative results in Fig.~\ref{fig:vis_vsnerf}, illustrating the superiority of our method over NeRF baselines in representing single scenes on challenging \textit{Coffee Cart} from Poly Haven and \textit{Entrée du château des Bois Francs} from Sketchfab.
Mesh2NeRF TensoRF supasses the original TensoRF, indicating that \OURS supervision contributes to the neural network's ability to learn accurate scene representation.
Mesh2NeRF NGP also outperforms Instant NGP, exhibiting fewer artifacts and providing more precise renderings.
For additional implementation details, results and analysis, please refer to the supplemental material.

\begin{table}[tb]
\centering
\vspace{-0.12in}
\caption{View synthesis results for fitting a single scene on ABO and Poly Haven datasets. Our comparison involves NeRF methods and \OURS, utilizing identical network architectures while differing in supervision style.
}
\vspace{-0.1in}
\scalebox{0.9}{
\begin{tabular}{lcccccc}
\Xhline{2\arrayrulewidth}
\multirow{2}{*}{Method}& \multicolumn{3}{c}{\textit{ABO Dataset}}   & \multicolumn{3}{c}{\textit{Poly Haven Dataset}}\\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
& \makebox[0.1\textwidth][c]{PSNR \textuparrow} & \makebox[0.1\textwidth][c]{SSIM \textuparrow} & 
\makebox[0.1\textwidth][c]{LPIPS \textdownarrow} & \makebox[0.1\textwidth][c]{PSNR \textuparrow} & \makebox[0.1\textwidth][c]{SSIM \textuparrow} & \makebox[0.1\textwidth][c]{LPIPS \textdownarrow} \\
\hline
NeRF & 25.09  & 0.882 & 0.137 & 21.24 & 0.689 & 0.422  \\
TensoRF  & 31.33& 0.944  & 0.032  & 23.32 & 0.748 & 0.260   \\
Instant NGP  & 30.16 & 0.928 & 0.039  & 24.39 & 0.779 & 0.185  \\
\hline
\OURS NeRF  & 32.40
& 0.942
& 0.044
& 22.75 & 0.710 & 0.296 \\
\OURS TensoRF  & 32.00
& 0.957  
& 0.024  
& 23.97 & 0.761 & 0.220 \\
\OURS NGP  & 
\textbf{33.28} 
& \textbf{0.969}
& \textbf{0.018}
&  \textbf{25.30}  
& \textbf{0.825}
& \textbf{0.129}
\\
\Xhline{2\arrayrulewidth}
\end{tabular}
}
\vspace{-0.15in}
\label{tab:single_object_results}
\end{table}




\subsection{Conditional Generation}
\label{subsec:cond_generation}
This section presents experimental results of NeRF generation conditioned on images of unseen objects from the ShapeNet Cars and Chairs~\cite{chang2015shapenet}, as well as the KITTI Cars~\cite{geiger2012we}.
These datasets pose unique challenges, with the ShapeNet Cars set featuring distinct textures, the ShapeNet Chair set exhibiting diverse shapes, and KITTI Cars representing real-world inference data with a substantial domain gap when compared to the training data of the generative model.

\mypara{Implementation information}
We adopt SSDNeRF~\cite{ssdnerf} as the framework for sparse-view NeRF reconstruction tasks since it achieves state-of-the-art NeRF generation performance.
In its single-stage training, SSDNeRF jointly learns triplane features of individual scenes, a shared NeRF decoder, and a triplane diffusion prior. 
The optimization involves a pixel loss from known views. 
For \textit{Ours}, we replace the pixel loss with 
Mesh2NeRF supervision (Eq.~\ref{eq:mesh2nerf_loss}) from the train set meshes. 
We generate training data for ShapeNet Cars and Chairs using the same lighting and mesh processes as in our Mesh2NeRF setup. 
SSDNeRF is trained using the official implementation; our model is trained with the same viewpoints as in the SSDNeRF experiments, without additional ray sampling, ensuring a fair comparison.
Our evaluation primarily centers on assessing the quality of novel view synthesis based on previously unseen images.
PSNR, SSIM, and LPIPS are evaluated to measure the image quality. 

\begin{figure*}[t!]
\vspace{-0.12in}
\centering
\includegraphics[width=1.0\textwidth]{AuthorKit/figures/ours_vs_ssdnerf.jpg}
\vspace{-0.23in}
\caption{Qualitative comparison of NeRF generation conditioned on single-view for unseen objects in ShapeNet Cars and Chairs between SSDNeRF and our method.  
Our approach enables more accurate novel views.
}
\vspace{-0.2in}
\label{fig:ssdnerf_single}
\end{figure*}

\mypara{Comparative evaluation} 
In Table~\ref{tab:spare-view}, a comprehensive comparison between our method and the state-of-the-art SSDNeRF is provided. Our method demonstrates overall superiority in conditional NeRF reconstruction tasks when provided with sparse-view conditions (ranging from one to four views) for both the Car and Chair categories.
Fig.~\ref{fig:ssdnerf_single} visually illustrates the impact of \OURS supervision on the accuracy of NeRFs in the context of single-view condition generation.
Notably, our method outperforms SSDNeRF, especially when dealing with objects that possess unconventional forms (e.g., the first car with a roof of the same color as the background, and the third red car exhibiting input noise). SSDNeRF struggles in such scenarios, yielding unreasonable geometries.
Qualitative comparisons in the setting of 2-view conditions are presented in both Fig.~\ref{fig:2view_condition}. In these scenarios, our approach consistently outshines SSDNeRF, producing superior results across various instances.

\begin{table}[tb!]
\caption{Conditional NeRF generation results on ShapeNet Cars and Chairs. We compare novel view synthesis outcomes conditioned on sparse views, ranging from one to four. \OURS{} consistently demonstrates superior performance compared to the state-of-the-art SSDNeRF.
} 
\vspace{-0.2in}
\begin{center}
\scalebox{0.71}{%
\setlength{\tabcolsep}{0.60em}
\begin{tabular}{lcccccccccccc}
\toprule
& \multicolumn{3}{c}{Cars 1-view} & \multicolumn{3}{c}{Cars 2-view} & \multicolumn{3}{c}{Cars 3-view} & \multicolumn{3}{c}{Cars 4-view} \\
\cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
& \makebox[0.07\textwidth]{PSNR \textuparrow} & \makebox[0.07\textwidth]{SSIM \textuparrow} & \makebox[0.07\textwidth]{LPIPS \textdownarrow} & \makebox[0.07\textwidth]{PSNR \textuparrow} & \makebox[0.07\textwidth]{SSIM \textuparrow} & \makebox[0.07\textwidth]{LPIPS \textdownarrow} & \makebox[0.07\textwidth]{PSNR \textuparrow} & \makebox[0.07\textwidth]{SSIM \textuparrow} & \makebox[0.07\textwidth]{LPIPS \textdownarrow} & \makebox[0.07\textwidth]{PSNR \textuparrow} & \makebox[0.07\textwidth]{SSIM \textuparrow} & \makebox[0.07\textwidth]{LPIPS \textdownarrow} \\
\midrule
SSDNeRF & 21.09 & 0.881 & 0.104 & 24.67 &  0.926 & \textbf{0.071}  & 25.71 & 0.934 & 0.069 & \textbf{26.54} & 0.939 & 0.067 \\
Ours & \textbf{21.78} & \textbf{0.893} & \textbf{0.101} & \textbf{24.98} & \textbf{0.932} & 0.072 & \textbf{25.89} & \textbf{0.942} & \textbf{0.066} & 26.51 & \textbf{0.945} & \textbf{0.062} \\
\midrule
 & \multicolumn{3}{c}{Chairs 1-view} & \multicolumn{3}{c}{Chairs 2-view} & \multicolumn{3}{c}{Chairs 3-view} & \multicolumn{3}{c}{Chairs 4-view}\\
 \cmidrule(lr){2-4}
\cmidrule(lr){5-7}
\cmidrule(lr){8-10}
\cmidrule(lr){11-13}
& \makebox[0pt]{PSNR \textuparrow} & \makebox[0pt]{SSIM \textuparrow} & \makebox[0pt]{LPIPS \textdownarrow}  & \makebox[0pt]{PSNR \textuparrow} & \makebox[0pt]{SSIM \textuparrow} & \makebox[0pt]{LPIPS \textdownarrow}  & \makebox[0pt]{PSNR \textuparrow} & \makebox[0pt]{SSIM \textuparrow} & \makebox[0pt]{LPIPS \textdownarrow}  & \makebox[0pt]{PSNR \textuparrow} & \makebox[0pt]{SSIM \textuparrow} & \makebox[0pt]{LPIPS \textdownarrow}\\
\midrule
SSDNeRF & 19.05 &  0.853 & 0.133 & 19.65 & 0.859 & 0.136 & 20.42 & 0.863 & 0.149 & 21.84 & 0.884 & 0.134 \\
Ours & \textbf{19.62} & \textbf{0.859} & \textbf{0.128} & \textbf{22.22} & \textbf{0.888} & \textbf{0.112} & \textbf{23.03} & \textbf{0.900} & \textbf{0.116} & \textbf{22.68} & \textbf{0.907} & \textbf{0.109}\\
\bottomrule
\end{tabular}
}
\end{center}
\label{tab:spare-view}
\vspace{-0.1in}
\end{table}


\begin{figure*}[th]
\centering
\includegraphics[width=1.02\textwidth]{AuthorKit/figures/recon2v_eccv.jpg}
\vspace{-0.15in}
\caption{Qualitatively comparison of NeRF generation conditioned on two-view for unseen objects in ShapeNet Cars and Chairs. Three novel views are displayed for each two-view input. Our approach enables more accurate novel views.}
\vspace{-0.15in}
\label{fig:2view_condition}
\end{figure*}






\mypara{Single-View NeRF Generation from Real Images} 
We also conduct a comparison with SSDNeRF using real KITTI car data for conditional generation based on a single-view input. 
This task poses a challenge because the generative model is trained on synthetic ShapeNet cars, resulting in a significant domain gap. 
The input images are obtained from the KITTI 3D object detection dataset~\cite{geiger2012we} using annotated 3D bounding boxes. To align them with the ShapeNet Cars dataset, we utilize provided bounding box dimensions and poses. Segmentation masks remove the background~\cite{heylen2021monocinis}. Images are cropped and resized to $128\times128$.
The processed image conditions our generative model, guiding the generation of a radiance field for rendering novel views around the cars.
In Fig.~\ref{fig:kitti}, we show qualitative examples of novel view synthesis.
Both SSDNeRF and our model successfully reconstruct the car's shape in most cases.
However, SSDNeRF fails in the last row sample due to color similarity between the car and the background. Our model excels in reconstructing the radiance field of the car in this challenging scenario. 
Regarding the generated car NeRFs, our approach produces more accurate textures with improved global consistency and better correspondence to the input image.
In contrast, SSDNeRF tends to generate textures only in the vicinity of the observation area, leaving other regions textureless or with incorrect colors. 
Our results exhibit greater realism and coherence across the entire scene, showcasing the superior generalization capability of our model, especially in the face of substantial domain gaps.


\begin{figure*}[t!]
\vspace{-0.05in}
\centering
\includegraphics[width=1\textwidth]{AuthorKit/figures/KITTI-CARS.jpg}
\vspace{-0.18in}
\caption{Qualitative comparison of novel view synthesis on in-the-wild car images from the KITTI dataset. Four novel views are displayed for each single-view input. Our approach enables more reasonable novel views.
}
\vspace{-0.1in}
\label{fig:kitti}
\end{figure*}

\subsection{Unconditional Radiance Field Synthesis}
\label{subsec:uncond_generation}
We conduct evaluation for unconditional generation using the Objaverse Mugs collection~\cite{deitke2023objaverse}, which consists of 153 mug models. 
The Mugs dataset presents a challenge in generating shape geometry and realistic textures due to the limited training samples. 
The baseline SSDNeRF is trained on rendered images from 50 views of each mesh, and \OURS is trained on meshes with the same viewpoints.
Both models underwent training for 100,000 iterations.

As shown in Fig.~\ref{fig:uncond_mugs}, both SSDNeRF and \OURS generate reasonable NeRFs in the rendered images.
However, when extracting meshes from NeRFs of SSDNeRF, inaccuracies are evident; the geometries of its unconditional generation do not faithfully represent the real geometry of the training samples or real data. 
Notably, traditional NeRF supervision struggles to enable the generative model to capture precise geometric details, such as whether a cup is sealed.
In contrast, \OURS synthesizes diverse and realistic geometries corresponding to the rendered images. 
This underscores the robustness of \OURS supervision, proving instrumental in generating physically plausible 3D content. 


\begin{figure*}[t!]
\vspace{-0.1in}
\centering
\includegraphics[width=1\textwidth]{AuthorKit/figures/Uncond_mugs.jpg}
\vspace{-0.25in}
\caption{Qualitative comparison between unconditional generative models training on Objaverse Mugs. We present two renderings and extracted mesh from each generated NeRF. Our approach exhibits a notable advantage in reasonable geometry, particularly for shapes that suffer from self-occlusions when trained only with image supervision.
}
\vspace{-0.2in}
\label{fig:uncond_mugs}
\end{figure*}


\subsection{Limitations}
While \OURS effectively employs direct NeRF supervision for NeRF representation and generation tasks, several limitations persist. 
Similar to NeRF, which bakes lighting information into appearance, we model the result of the Phong lighting
model in the generated radiance field for compatibility with existing approaches.
Another limitation stems from the ray sampling employed by baselines due to the dependence on rendered images. Hence, future work should delve into more efficient sampling techniques that leverage ground truth geometry and appearance, bypassing the need for sampling schemes relying on virtual cameras. 
Furthermore, acknowledging the diversity of mesh data, the application of Mesh2NeRF to generative models can span across various categories of mesh data, contributing to the development of a more universal and robust prior.
